Learning the Structure of Large Networked Systems Obeying Conservation Laws

Many networked systems such as electric networks, the brain, and social networks of opinion dynamics are known to obey conservation laws. Examples of this phenomenon include the Kirchoff laws in electric networks and opinion consensus in social networks. Conservation laws in networked systems may be modeled as balance equations of the form $X = B^{*} Y$, where the sparsity pattern of $B^{*}$ captures the connectivity of the network, and $Y, X \in \mathbb{R}^p$ are vectors of "potentials" and "injected flows" at the nodes respectively. The node potentials $Y$ cause flows across edges and the flows $X$ injected at the nodes are extraneous to the network dynamics. In several practical systems, the network structure is often unknown and needs to be estimated from data. Towards this, one has access to samples of the node potentials $Y$, but only the statistics of the node injections $X$. Motivated by this important problem, we study the estimation of the sparsity structure of the matrix $B^{*}$ from $n$ samples of $Y$ under the assumption that the node injections $X$ follow a Gaussian distribution with a known covariance $\Sigma_X$. We propose a new $\ell_{1}$-regularized maximum likelihood estimator for this problem in the high-dimensional regime where the size of the network $p$ is larger than sample size $n$. We show that this optimization problem is convex in the objective and admits a unique solution. Under a new mutual incoherence condition, we establish sufficient conditions on the triple $(n,p,d)$ for which exact sparsity recovery of $B^{*}$ is possible with high probability; $d$ is the degree of the graph. We also establish guarantees for the recovery of $B^{*}$ in the element-wise maximum, Frobenius, and operator norms. Finally, we complement these theoretical results with experimental validation of the performance of the proposed estimator on synthetic and real-world data.

==> Web_links.tex <==
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7953282
https://n.neurology.org/content/neurology/89/13/1373.full.pdf
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9369883
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7551715
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8700659
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8008816
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7990048
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7450694
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7742951
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8646701
https://www.sciencedirect.com/science/article/pii/S0165168421001870
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7472541
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9244648
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7383833
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8335493
https://epubs.siam.org/doi/pdf/10.1137/19M1263340
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7472448
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8462154
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9090980
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7952928
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7472448
https://reader.elsevier.com/reader/sd/pii/S0165168421002188?token=3E063B34AB27ECB468C55406B6A9CB0AF78E24E31BADC09604F94037A8C1CEC46E523DD6817BC007621FD62607832BF2&originRegion=us-east-1&originCreation=20220510172718
http://cas.tudelft.nl/pubs/leus18graphchapter.pdf
https://arxiv.org/pdf/2109.11700.pdf
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9747524
http://www2.ece.rochester.edu/~gmateosb/pubs/netist/NETIST_BOOK.pdf
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8450838
https://ieeexplore.ieee.org/abstract/document/9497730

https://link.springer.com/content/pdf/10.1007/s10548-016-0538-7.pdf
https://link.springer.com/content/pdf/10.1007/s10548-016-0538-7.pdf
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=6736229

https://escholarship.org/content/qt1q6298g0/qt1q6298g0.pdf (statespace later)
https://web.wpi.edu/Pubs/ETD/Available/etd-032218-131000/unrestricted/TMReese.pdf
https://arxiv.org/pdf/1909.00853.pdf

%Tropp 
https://epubs.siam.org/doi/pdf/10.1137/090771806
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=1377501
https://link.springer.com/content/pdf/10.1007/s00211-021-01250-3.pdf
https://journals.aps.org/pre/pdf/10.1103/PhysRevE.102.042315
http://csnmbs.manu.edu.mk/index.php/csnmbs/article/viewFile/33/30
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7393962

